Examining User-Friendly and Open-Sourced Large GPT Models: A Survey on Language, Multimodal, and Scientific GPT Models

Generative pre-trained transformer (GPT) models have revolutionized the field of natural language processing (NLP) with remarkable performance in various tasks and also extend their power to multimodal domains. Despite their success, large GPT models like GPT-4 face inherent limitations such as considerable size, high computational requirements, complex deployment processes, and closed development loops. These constraints restrict their widespread adoption and raise concerns regarding their responsible development and usage. The need for user-friendly, relatively small, and open-sourced alternative GPT models arises from the desire to overcome these limitations while retaining high performance. In this survey paper, we provide an examination of alternative open-sourced models of large GPTs, focusing on user-friendly and relatively small models that facilitate easier deployment and accessibility. Through this extensive survey, we aim to equip researchers, practitioners, and enthusiasts with a thorough understanding of user-friendly and relatively small open-sourced models of large GPTs, their current state, challenges, and future research directions, inspiring the development of more efficient, accessible, and versatile GPT models that cater to the broader scientific community and advance the field of general artificial intelligence. The source contents are continuously updating in https://github.com/GPT-Alternatives/gpt_alternatives.

==> Table/2_longtable.tex <==
\clearpage
\onecolumn

\begin{longtable}{l|p{0.3 \columnwidth}|l|l|p{0.3 \columnwidth}}  
\caption{Statistics of open large language models in recent years categorized by the base models.}
\label{tab:cc} \\
\toprule
Model & \#Param & Backbone & Release Date & Training Data \\
\midrule
T5~\cite{raffel2020exploring} & 60M, 220M, 770M, 3B, 11B & Base Model & 2019-10 & C4~\cite{raffel2020exploring}, 1T tokens \\
\midrule
mT5~\cite{xue2020mt5}  & 300M, 580M, 1.2B, 3.7B, 13B & Base Model & 2020-10 & mC4, 1T tokens \\
\midrule
GPT-Neo~\cite{gpt-neo} & 125M, 350M, 1.3B, 2.7B & Base Model & 2021-03 & the Pile~\cite{gao2020pile}, 825GB \\
\midrule
GPT-J~\cite{gpt-j} & 6B & Base Model & 2021-06 & the Pile~\cite{gao2020pile}, 825GB \\
\midrule
GPT-NeoX~\cite{black2022gpt} & 20B & Base Model & 2022-02 & the Pile~\cite{gao2020pile}, 825GB \\
\midrule
OPT~\cite{zhang2022opt} & 125M, 1.3B, 2.7B, 6.7B, 13B, 30B, 66B, 175B & Base Model & 2022-05 &  Pile~\cite{gao2020pile} and d PushShift.io Reddit~\cite{baumgartner2020pushshift}, 180B tokens \\
\midrule
Bloom~\cite{scao2022bloom} & 560M, 1.1B, 1B7, 3B, 7.1B, 176B & Base Model & 2022-07 & ROOTS corpus~\cite{laurenccon2022bigscience}, 366B tokens \\
BloomZ & 560M, 1.1B, 1B7, 3B, 7.1B, 176B & Bloom & 2022-11 & xP3(extended from P3~\cite{sanh2021multitask}) \\
\midrule
GLM~\cite{du2022glm, zeng2023glm-130b} & 110M, 335M, 410M, 515M, 2B, 10B, 130B & Base Model & 2021-03, 2022-08 & BooksCorpus~\cite{zhu2015aligning} and
English Wikipedia \\
ChatGLM & 6B & GLM & 2023-03 & unknown \\
\midrule
LLaMA~\cite{touvron2023llama} & 7B, 13B, 33B, 65B & Base Model & 2023-02 & English CommonCrawl, C4~\cite{raffel2020exploring}, Github, Wikipedia, Gutenberg Books3 and Stack Exchange, 1.4T tokens \\
OpenLLaMA~\cite{openlm2023openllama} & 3B, 7B & Replicate of LLaMA & 2023-05 & \\
Alpaca~\cite{alpaca} & 7B & LLaMA & 2023-03 & 52K data generated from text-davinci-003 \\
Vicuna~\cite{vicuna} & 7B, 13B & LLaMA & 2023-03 & 70K user-shared conversations from ShareGPT \\
StableVicuna~\cite{stablelm} & 13B & LLaMA \& Vicuna & 2023-04 & - \\
BAIZE~\cite{xu2023baize} & 7B, 13B, 30B & LLaMA & 2023-04 & 54K/57K/47K dialogs from Quora, StackOverFlow and MedQuAD questions \\
Koala~\cite{koala_blogpost_2023} & 13B & LLaMA & 2023-04 & A gather of ShareGPT\footnote{\url{https://sharegpt.com}}, HC3~\cite{guo2023close}, OIG\footnote{\url{https://laion.ai/blog/oig-dataset}}, Stanford Alpaca~\cite{alpaca}, Anthropic HH\footnote{\url{https://huggingface.co/datasets/Anthropic/hh-rlhf}}, OpenAI WebGPT~\cite{nakano2021webgpt}, and OpenAI Summarization~\cite{stienon2020learning} \\
WizardLM~\cite{xu2023wizardlm} & 7B, 13B, 30B & LLaMA & 2023-06 &  250k evolved instructions (from ShareGPT)/70k evolved instructions (from Alpaca~\cite{alpaca} data) \\
UltraLM~\cite{ding2023ultralm} & 13B & LLaMA & 2023-06 & UltraChat~\cite{UltraChat} \\
\midrule
Pythia~\cite{biderman2023pythia} & 70M, 160M, 410M, 1B, 1.4B, 2.8B, 6.9B, 12B & Base Model & 2023-01 & the Pile~\cite{gao2020pile}/the Pile with deduplication applied, 299.9B tokens/207B tokens \\
Dolly-v2~\cite{dolly} & 12B & Pythia & 2023-04 & \textasciitilde 15k instruction/response finetuning records \\
Openchatkit~\cite{openchatkit} & 7B & Pythia & 2023-03 & the OIG\footnote{\url{https://laion.ai/blog/oig-dataset/}} dataset \\
BELLE-7B~\cite{belle} & 7B & Pythia & 2023-03 & 1.5M Chinese Dataset\footnote{\url{https://github.com/LianjiaTech/BELLE/tree/main/data/1.5M}} \\
\midrule
StableLM~\cite{stablelm} & 3B, 7B & Base Model & 2023-04 & dataset that build on the Pile~\cite{gao2020pile}, 1.5T tokens \\
StableLM-Tuned-Alpha~\cite{stablelm} & 7B & StableLM & 2023-04 & Stanford's Alpaca, Nomic-AI's gpt4all, RyokoAI's ShareGPT52K datasets, Databricks labs' Dolly, and Anthropic's HH \\
\midrule
RWKV~\cite{peng2023rwkv} & 169M, 430M, 1.5B, 3B, 7B, 14B & Base Model & & the Pile~\cite{gao2020pile} \\
ChatRWKV~\cite{chatrwkv} & 7B, 14B & RWKV & 2022-12 &  \\
\midrule
moss-moon-003-base~\cite{moss} & 16B &  & 2023-04 & 700B tokens \\
moss-moon-003-sft~\cite{moss} & 16B &  & 2023-04 & 1.1 million multi-round conversational data \\
\midrule
RedPajama-INCITE~\cite{RedPajama-INCITE} & 3B, 7B & Base Model & 2023-05 & RedPajama-Data~\cite{redpajama-data}, 1.2T tokens \\
\midrule
MPT-7B~\cite{mpt7b}  & 7B & Base Model & 2023-05 & 1T tokens \\
MPT-7B-Chat & 7B & MPT-7B & 2023-05 &  ShareGPT-Vicuna, HC3, Alpaca, Helpful and Harmless, and Evol-Instruct datasets \\
\midrule
Falcon LLM & 7B, 40B & Base Model & 2023-06 & \\
\bottomrule
\end{longtable} 

\clearpage
\twocolumn
